Hardware-based Security for Virtual Trusted Platform Modules

Virtual Trusted Platform modules (TPMs) were proposed as a software-based alternative to the hardware-based TPMs to allow the use of their cryptographic functionalities in scenarios where multiple TPMs are required in a single platform, such as in virtualized environments. However, virtualizing TPMs, especially virutalizing the Platform Configuration Registers (PCRs), strikes against one of the core principles of Trusted Computing, namely the need for a hardware-based root of trust. In this paper we show how strength of hardware-based security can be gained in virtual PCRs by binding them to their corresponding hardware PCRs. We propose two approaches for such a binding. For this purpose, the first variant uses binary hash trees, whereas the other variant uses incremental hashing. In addition, we present an FPGA-based implementation of both variants and evaluate their performance.

==> figures/tikz-incremental-hashing-datapath.tex <==
\begin{tikzpicture}

% Register
\node [shape=reg] (pcrold) {$PCR_{old}$};
\node [shape=reg,right=of pcrold] (sibling) {$sibling_i$};
\node [shape=reg,right=of sibling] (pcrnew) {$PCR_{new}$};

% Muxes
\node [mux,above=of pcrold,rotate=180] (oldinput) {};
\node [mux,above=of pcrnew,rotate=180] (newinput) {};

% Input names
\node [above=of oldinput.205,yshift=-.5cm] (old){$PCR_{old}$};
\node [above=of newinput.335,yshift=-.5cm] (new){$PCR_{new}$};
\node [above=of sibling,yshift=.5cm] (sibl) {$sibling_i$};

% Hash functions
\node [myrect,below=of pcrold.335,xshift=.5cm] (hashold) {SHA-1};
\node [myrect,below=of pcrnew.205,xshift=-.5cm] (hashnew) {SHA-1};

% PCR'
\node [below=of hashold] (oldprime) {$PCR'_{old}$};
\node [below=of hashnew] (newprime) {$PCR'_{new}$};

%%%%%%%%%%
% Arrows %
%%%%%%%%%%
% Inputs
\draw [->] (old) -- (oldinput.205);
\draw [->] (new) -- (newinput.335);
\draw [->] (sibl) -- (sibling);

% feedback
\draw [->] (hashold.south) |- ++(-3,-.4) |- ($(oldinput.335) + (0,.4)$) -| (oldinput.335);
\draw [->] (hashnew.south) |- ++(3,-.4) |- ($(newinput.205) + (0,.4)$) -| (newinput.205);

\draw [->] (oldinput) -- (pcrold);
\draw [->] (newinput) -- (pcrnew);

\draw [->] (pcrold) |- ($(hashold.135) + (0,.4)$) -- (hashold.135);
\draw [->] (pcrnew) |- ($(hashnew.45) + (0,.4)$) -- (hashnew.45);

\draw [->] (sibling.240) |- ($(hashold.45) + (0,.5)$) -| (hashold.45);
\draw [->] (sibling.300) |- ($(hashnew.135) + (0,.5)$) -| (hashnew.135);

\draw [->] ($(hashold.south) + (0,-.4)$) -- (oldprime);
\draw [->] ($(hashnew.south) + (0,-.4)$) -- (newprime);

\end{tikzpicture}


==> hashing.tex <==
\section{Approach}
\label{sec:approach}

\todo{SM}{remove this subsection and add this text in approach}

Currently available TPMs are not capable of handling hash trees thus we present our novel approaches as described in the follwing.
The fundamental idea behind providing the hardware-based security to a virtual machine is based on computing the root hash value.
The root hash value is the combined hash value of the multiple virtual PCRs (vPCRs)and is stored in the hardware PCR.
The vPCRs of the vTPM are bound in such a way that any modification to them can be detected.
To compute these values and bind (map) them to the hardware PCRs, we use two approaches: Hash Tree based Binding and Incremental Hash based Binding.


In a virtualization scenario, during the setup of the dom0 (hypervisor) the height of the hash tree, represented by an internal counter, is fixed and the TPM will be initialized accordingly.
The TPM needs to maintain only three values to be able to verify an update of the hash tree. \todo{SM}{which three: old, new, and intermediate?}
The tree update consists of two operations: $TPM\_update\_leaf$ and $TPM\_update\_intermediate$.
If the update\_leaf function is called, the TPM stores the supplied old PCR value ($PCR_{old}$) and the new PCR value ($PCR_{new}$).
The intermediate values needed to recompute the hash tree are transmitted to the TPM iteratively as a parameter of the update\_intermediate function in each iteration.
For each function call, the internal counter is decremented by one and when the counter reaches zero the result of the hash function is compared with the stored value in the corresponding PCR register.
If the $PCR_{old}$ matches the stored state in the TPM's hardware PCR, it is updated with $PCR_{new}$, which has been computed in parallel to the aforementioned verification process.
Further, the new hash values stored in the $PCR_{new}$ register are sent to the Trusted Software Stack (TSS) after completion of the tree update.


\todo{SM}{insert the following after approach}

%----------------------------------%
\subsection{Hash Tree Based Binding}
%----------------------------------%

The hash tree based binding approach makes use of the well-known binary hash trees as shown in Figure~\ref{fig:hash_tree}.
This approach consits of three phases: the setup phase, the integrity measurement phase, and the remote attestation phase.

%------------------%
%%% Hash Tree %%%
%------------------%
\begin{figure}
\centering
\resizebox{0.8\columnwidth}{!}{\begin{tikzpicture}[level/.style={sibling distance=50mm/#1}]
\begin{scope}[grow=up]
\node [circle,draw] (z){$h_0$}
  child {node [circle,draw] (a) {$h_2$}
    child {node [circle,draw] (b) {$h_6$}
      child {node {$\vdots$}
        child {node [rectangle,draw,xshift=3mm] (d) {$vPCR_i^n$}}
        child {node [rectangle,draw,xshift=-3mm] (e) {$vPCR_i^{n-1}$}}
      } 
      child {node {$\vdots$}}
    }
    child {node [circle,draw] (g) {$h_5$}
      child {node {$\vdots$}}
      child {node {$\vdots$}}
    }
  }
  child {node [circle,draw] (j) {$h_1$}
    child {node [circle,draw] (k) {$h_4$}
      child {node {$\vdots$}}
      child {node {$\vdots$}}
    }
    child {node [circle,draw] (l) {$h_3$}
      child {node {$\vdots$}}
      child {node (c){$\vdots$}
        child {node [rectangle,draw,xshift=2mm] (o) {$vPCR_i^2$}}
        child {node [rectangle,draw,xshift=-2mm] (p) {$vPCR_i^1$}}
      }
    }
  };
\end{scope}

\path (a) -- (j);
\path (b) -- (g);
\path (k) -- (l);
\path (k) -- (g);
\path (d) -- (e);
\path (o) -- (p);
\path (o) -- (e) node (x) [midway] {$\cdots$};
\end{tikzpicture}
}
\caption{Sample Binary Hash Tree}
\label{fig:hash_tree}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Setup Phase}
%%%%%%%%%%%%%%%%%%%%%%%
The leaves at the top of the tree represent all vPCRs of a specific index~$i$ of all existing vTPMs ($1,\ldots,n$). 
We assume that the number of leaves equals the number of the VMs existing on this platform.
\todo{TF}{really needed? We supply the height of the tree with the recalculation process. In order to get the right result the height has to be correct, else this would result in finding a collision.}
In our approach, we propose using pre-computed hash trees of height $l$ to gain more efficiency i.e., with $l=10$, one can run 1024 vTPMs on the same platform bound to the hardware TPM.
%that can be bound to the hardware TPM to provide more security. This number is --- in fact --- not imaginable number for single platforms~(e.g., Servers).
Nodes further up in the tree are the hash values of their respective child nodes leading to the root hash at the top (bottom?) of the tree.

Applying the description to Figure~\ref{fig:hash_tree} shows that $h_0$ represents the value of the PCR of index $i$ ($PCR_i$) of the hardware TPM.
$h_0$ is obtained by combining the hashes $h_1$ and $h_2$, i.e.,
\begin{equation*}
h_0 \Leftarrow  hash(h_1 || h_2), 
\end{equation*}
where $||$ indicates the concatenation operation.\\
Similar to $h_0$, all intermediate hashes are computed. 
Thus, the calculation of $h_0$ depends on the the leaves and all intermediate nodes of the hash tree.

%Consequentially, any unauthorized modification to one of the leaves~(i.e. vPCRs) can be detected. (repeated?)
%The hash h0 is stored in the PCR0 of the hardware TPM, thus mapping the vTPM instances to the hardware TPM.
%The root hashes for all other PCRs of the VMs are computed using the hash tree and are stored in corresponding PCRs inside the hardware TPM.
%Thus, our approach is more secure than the vTPM approach \cite{vtpm} because the platform state is now stored inside the hardware TPM which is more difficult to attack. 

%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Integrity Measurement}
%%%%%%%%%%%%%%%%%%%%%%

As mentioned before, we assume that all integrity measurement modules are trusted and behave correctly.
That is, for a given VM, new measurements are reported to the vTPM associated with it with the assumption that every loaded executable is measured correctly.
After a measurement is computed, the vTPM is notified about the new measurement to extend the value of a specific vPCR and corresponding SML is also updated.
%In addition, the SML of this vTPM is also updated. 
Since we assume that vTPMs can be attacked, an attacker can modify the newly extended value to another value, which is trusted by the challenger. 
The SML of the attacked vTPM can also be changed accordingly but to avoid this, the new extended value of the vTPM is bound to the hardware TPM. 
With this, modifications at a later time to any of the vPCRs can be detected. 
We achieve this by using hash trees, making the value of hardware PCR of index $i$ dependent on the values of all existing vPCRs of the same index $i$.
In our approach, a change in the state of any VM, for example after loading a new application, causes re-calculating the hash tree which in turn results in a new root hash.

More specifically, the TSS notifies the underlying hardware TPM about the loaded application by starting the procedure depicted in Algorithm~\ref{alg:hashStart}.
The inputs to the algorithm are the old vPCR value $vPCR_{old}$, the new vPCR value $vPCR_{new}$, the height of the hash tree $l$, and the PCR index $i$ of the hardware TPM. 
This algorithm is then executed inside the hardware TPM, which in turn stores the generated values in temporary registers in the volatile storage.
The algorithm returns "OK" if and only if the storing process was successfully finished and there is no hash tree updating process running for this $PCR_i$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\KwIn{old vPCR value $vPCR_{old}$,\\ new vPCR value $vPCR_{new}$,\\ hardware PCR index $PCR_i$,\\ height of the tree $l$}
\KwOut{updated $PCR'_{new}$}
\If(\tcp*[f]{a hash tree execution is running}){$c_i \neq 0$}{
	\Return error\;
}
\Else{
  $c_i \gets l$ \tcp*[f]{initialize counter with tree height}
  $tmp_{old} \gets vPCR_{old}$\;
  $tmp_{new} \gets vPCR_{new}$\;
}
\caption{\label{alg:hashStart} starting the hash tree execution}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\KwIn{hardware PCR index $PCR_i$, sibling}
\KwOut{updated root PCR $PCR'_{new}$.}
$tmp_{old} = hash(tmp_{old}||sibling)$\;
$tmp_{new} = hash(tmp_{new}||sibling)$\;
$c_i \gets c_i-1$\;
\If(\tcp*[f]{root of tree reached}){$c_i = 0$}{
\If{$tmp_{old} = PCR_i$}{
$PCR_i \gets tmp_{new}$\;
\Return $PCR_{new}$\;
}
\Else{
\Return $error$; \tcp*[f]{the hash tree is tampered}\
}}

\caption{\label{alg:hashUpdate} updating the hash tree and the root}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\todo{SM} {it is redundant}
After providing the hardware TPM with the old and new vPCR values, the re-calculation of the hash tree can be executed as shown in Algorithm~\ref{alg:hashUpdate}.
Since the hash tree is located outside of the TPM and the algorithm must be provided with all siblings located in the traverse path to the root of the hash tree, Algorithm~\ref{alg:hashUpdate} must be called
$l-1$ times, providing at each time the correct sibling of the current hash tree level. 
First, the TPM is provided with the sibling of the leaf (i.e., the vPCR) and hashes the old and the new value of the vPCR with its sibling. 
The same process is repeated until the root is reached (i.e., the tree height = 0).
If now the old vPCR value equals the value stored in $PCR_i$, this means that the hash tree is untampered and the new calculated root can be stored in $PCR_i$ \todo{SA}{discuss overwrite or extend?},
otherwise an error is returned. 
It does not matter who calls Algorithm~\ref{alg:hashUpdate} in the hardware TPM to provide the siblings values, more important is the provision of the correct values to calculate a correct root value, which equals $PCR_i$.
That is, an attacker which calls Algorithm~\ref{alg:hashUpdate} after the Algorithm~\ref{alg:hashStart} was called, would not win anything.

Note that it would be possible to provide the TPM with all required siblings (from a leaf to the root) at once. 
Although this would reduce the communication overhead occuring as described above, it requires the presence of enough temporary registers for all these values, which could be a problem for resource constraint devices, like the TPM.

%%%%%%%%%%%%%%%%%%%%
\paragraph{Remote Attestation}
The remote attestation process is very similar to the one described by TCG, with an additional task of verifying the hash tree.
After sending a nonce and signing it and the requested vPCR by a vAIK of a particular vTPM, the nonce is then forwarded to the hardware TPM. 
The hardware TPM also signs the nonce and the value of the requested PCR. 
These signatures, the SML and the hash tree are then sent to the challenger. 
The challenger verifies the correctness of the signatures and the SML in addition to re-calculating the hash tree as described above. 
If the signed root value equals the re-calculated value, it means that the vPCR is untampered and can be trusted.

%Remote attestation is one of the main functions provided by the TPM, where in the attester trustworthily reports his platform status to a remote challenger.
%For this, a digital signature is computed for the Attestation Identity Key (AIK) by the privacy certification authority (a trusted third party).
%AIK is an asymmetric session key from the attester, which can be validated later with the help of a trusted third party by providing the AIK certificate.
%The private part of this AIK is used for signing the PCRs, which are sent to the challenger along with the SML and the AIK certificate.
%The challenger takes the PCR values and the AIK certificate for verifying trustworthiness of the system and to establish the communication with the attester.
%This section compares the vTPM based approach with our proposed novel approach with respect to remote attestation.
%
%The remote attestation procedure with vTPM based approach is similar to the standard procedure defined by TCG.
%When a customer requests for an attestation to the vTPM on his allocated VM, he is provided with vPCRs representing the state of his VM and the SML.
%Firstly he verifies the signature of the obtained PCR values from the attester.
%Secondly he recomputes the hash values form the SML of the vTPM.
%The trustworthioness of the system is checked by comparing the computed hash value with the obtained hash value form the attester.
%However because the hardware PCRs are replaced with virtual PCRs (software PCRs) they can be maliciously modified by the attacker.
%Further the SML is also modified to falsify the challenger about the trustworthiness of the allocated VM.
%
%In contrast, with our proposed approach an additional vefification step is included in the standard remote attestation procedure to overcome the above mentioned drawback.
%When a customer requests for an attestation to the vTPM, he is provided with the root hash (by a TTP) and intermediate hashes of the hash tree, in addition to vPCRs representing the state of his VM and the SML.
%The root hash in this case being stored in the hardware TPM, any malicious modifications by the attacker are detected while recalculating the root hash from SML and the intermediate hashes.
%With this approach the trustworthiness of the VM to the customer is guaranteed without knowing the state of the other VMs.
%This is because for other VMs only the hash values resulting form their state are provided but not their vPCRs.
%
%\todo{introduce merkle hash trees}\\
%\todo{applicability to our approach}\\
%\todo{advs and disadvs w.r.t add/del of VMs}\\
%


==> relatedWork.tex <==
\section{Related Work}


==> tc.tex <==
\subsection{Trusted Computing}
\label{sec:tc}
% The standards and specifications of Trusted Computing~\cite{TPM2011,?} provide many functionalities to secure computing platforms. 
% One of these functionalities is to build a chain of trust starting from a hardware trust anchor, called the Trusted Platform Module (TPM).
% The TPM is a hardware chip which provides the platform with cryptographic functions (such as hashing, encryption and decryption) as well as a secure and small storage.
% The chain is then extended by measuring every loaded component following the principle "hash then load" before passing control to it. 
% That is, the chain includes all loaded software on the platform. 
% To allow storing all these measurements in the small and secure storage inside the TPM, the measurements are concatenated and hashed using the SHA-1 hash. 
% The result is then always a 160-bit value, which can be stored in one of the provided registers, called Platform Configuration Registers (PCRs), inside the TPM.
% This value signals the state of the system.

Trusted Computing standard specifies a cryptographic module, called TPM \cite{TPM2011}, that provides various security functionalities.
TPM is a microcontroller-based chip with hard-wired engines for various cryptographic functions such as RSA, SHA-1 and HMAC.
It forms the trust anchor of a system by building whole chain-of-trust which includes all loaded software on the platform.
The chain is extended based on the principle \emph{hash then load} i.e., every loaded software is hashed using SHA-1 algorithm before passing control to it.
The computed hash values, representing the state of the system, are stored in Platform Configuration Registers (PCRs) of the TPM.

%\todo{TF}{define acronyms SML, VM, ...}

% Another important functionality of TC is the so-called remote attestation process. 
% In this process, the value stored in a PCR is reported in a secure manner to a challenger to allow him deciding on the trustworthiness of the platform by comparing it with well-known and trusted reference values stored in
% a list called the Reference Measurement List (RML).

Remote Attestation is one important security function provided by the TPM.
In remote attestation, the system with a TPM has to trustworthily report its platform status to a remote challenger.
For this, the TPM provides a set of PCR values signed by the Attestation Identity Key (AIK) and a Stored Measurement Log (SML) to the challenger.
In turn, the challenger decides on trustworthiness of the system by comparing them with the well-known refernce values stored in a public Reference Measurement List (RML)

% Unfortunately the current specification of the TPM does not provide a possibility to update or add new functionalities to the TPM. 
% However, TCG has released as set of requirements for the next generation of the TPM \cite{tpm.next}, which include requirements about possibilities of update and addition of new functionalities.
% Also researchers proposed the use of reconfigurable TPMs.
% For instance, TinyTPM~\cite{?} provides bla bla bla..
% \\
% \todo{SA}{Thomas binde bitte deinen Teil hier}

Unfortunately the current specification of the TPM does not support hardware-based security for systems using virtualization and cloud computing technologies.
Though there exist in literature, designs supporting resource constrained embedded systems \cite{tinyTPM} and arbitrary number of virtual TPMs \cite{vTPM2007}, they do not address the above problem.
Further, TCG has released a set of requirements in its next generation TPM specification \cite{tpm.next} to be considered for future TPMs.
With regard to above requirements, in this contribution we propose and implement methods to provide hardware-based security in aforementioned technologies.


% \paragraph{TPM}%May be removed later
% The TPM provides tamper resistant storage for storing the artifacts of the system.
% Special solutions for a variety of application scenarios of TPMs have been presented in literature.
% Ranging from resource constraint embedded systems with strict requirements on resource utilization (cf. \cite{tinyTPM}) to supporting arbitrary number of TPMs in large data center or cloud environments as presented in the vTPM approach \cite{vTPM2007}.
% The aforementioned integrity measurement and remote attestation schemes are supported by dedicated hardware-based cryptographic engines in the TPM.
% 
% The Trusted Computing Group has released as set of requirements for the next generation of the TPM \cite{tpm.next}.
% In addition to supporting new algorithms and their updatability, the support for virtualized system has to be considered for future TPMs. 
% 
% \todo{TF}{It is not clear to me what else you want to write here without generating redundancy}

